log-RRIM: Yield Prediction via Local-to-global Reaction Representation Learning and Interaction Modeling

Accurate prediction of chemical reaction yields is crucial for optimizing organic synthesis, potentially reducing time and resources spent on experimentation. With the rise of artificial intelligence (AI), there is growing interest in leveraging AI-based methods to accelerate yield predictions without conducting in vitro experiments. We present log-RRIM, an innovative graph transformer-based framework designed for predicting chemical reaction yields. A key feature of log-RRIM is its integration of a cross-attention mechanism that focuses on the interplay between reagents and reaction centers. This design reflects a fundamental principle in chemical reactions: the crucial role of reagents in influencing bond-breaking and formation processes, which ultimately affect reaction yields. log-RRIM also implements a local-to-global reaction representation learning strategy. This approach initially captures detailed molecule-level information and then models and aggregates intermolecular interactions. Through this hierarchical process, log-RRIM effectively captures how different molecular fragments contribute to and influence the overall reaction yield, regardless of their size variations. log-RRIM shows superior performance in our experiments, especially for medium to high-yielding reactions, proving its reliability as a predictor. The framework's sophisticated modeling of reactant-reagent interactions and precise capture of molecular fragment contributions make it a valuable tool for reaction planning and optimization in chemical synthesis. The data and codes of log-RRIM are accessible through https://github.com/ninglab/Yield_log_RRIM.

==> tables/different_pretraining.tex <==
\begin{table}[htbp]
\caption{Different pre-trained MAT weights usage strategy performance}
\label{tbl:different_pretraining_method}
\centering
\begin{threeparttable}
\begin{tabular}{    
    %
    @{\hspace{8pt}}c@{\hspace{8pt}}
    %
    @{\hspace{3pt}}c@{\hspace{3pt}}
    %
    @{\hspace{3pt}}c@{\hspace{3pt}}
    %
    @{\hspace{3pt}}c@{\hspace{3pt}}
     %   
     @{\hspace{3pt}}c@{\hspace{3pt}}
    %
    @{\hspace{3pt}}c@{\hspace{3pt}}
    %
    @{\hspace{3pt}}c@{\hspace{3pt}}
     %   
     @{\hspace{3pt}}c@{\hspace{3pt}}
    %
    @{\hspace{3pt}}c@{\hspace{3pt}}
    %
    @{\hspace{3pt}}c@{\hspace{3pt}}
    }
\toprule
Number of freezed layers $l$ & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8\\
\midrule
Test MAE & 0.0352 & 0.0353 & 0.0358 & 0.0361 & 0.0367 & 0.0381 & 0.0397 & 0.0392 & 0.0387 \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table}


